Equilibrium and Termination

We present a reduction of the termination problem for a Turing machine (in the simplified form of the Post correspondence problem) to the problem of determining whether a continuous-time Markov chain presented as a set of Kappa graph-rewriting rules has an equilibrium. It follows that the problem of whether a computable CTMC is dissipative (ie does not have an equilibrium) is undecidable.

==> eptcsdata.tex <==
\providecommand{\event}{S. B. Cooper, E. Kashefi, P. Panangaden (Eds.): Developments in\\ Computational Models (DCM 2010)}
\providecommand{\volume}{26}
\providecommand{\anno}{2010}
\providecommand{\firstpage}{75}
\providecommand{\eid}{7}
\pdfoutput=1

